NAWQ-SR: A Hybrid-Precision NPU Engine for Efficient On-Device Super-Resolution

In recent years, image and video delivery systems have begun integrating deep learning super-resolution (SR) approaches, leveraging their unprecedented visual enhancement capabilities while reducing reliance on networking conditions. Nevertheless, deploying these solutions on mobile devices still remains an active challenge as SR models are excessively demanding with respect to workload and memory footprint. Despite recent progress on on-device SR frameworks, existing systems either penalize visual quality, lead to excessive energy consumption or make inefficient use of the available resources. This work presents NAWQ-SR, a novel framework for the efficient on-device execution of SR models. Through a novel hybrid-precision quantization technique and a runtime neural image codec, NAWQ-SR exploits the multi-precision capabilities of modern mobile NPUs in order to minimize latency, while meeting user-specified quality constraints. Moreover, NAWQ-SR selectively adapts the arithmetic precision at run time to equip the SR DNN's layers with wider representational power, improving visual quality beyond what was previously possible on NPUs. Altogether, NAWQ-SR achieves an average speedup of 7.9x, 3x and 1.91x over the state-of-the-art on-device SR systems that use heterogeneous processors (MobiSR), CPU (SplitSR) and NPU (XLSR), respectively. Furthermore, NAWQ-SR delivers an average of 3.2x speedup and 0.39 dB higher PSNR over status-quo INT8 NPU designs, but most importantly mitigates the negative effects of quantization on visual quality, setting a new state-of-the-art in the attainable quality of NPU-based SR.

==> algorithms/nawqsr.tex <==

% Overall NAWQ-SR algorithm
\setlength{\textfloatsep}{0pt}
\SetArgSty{textnormal}
\begin{algorithm}[!t]
    \footnotesize
    \SetAlgoLined
    \LinesNumbered
    \DontPrintSemicolon
    \KwIn{DNN $m$ with layers $\mathcal{L}$}
    \nonl
    \myinput{Wordlengths set $\mathcal{W}=\{8,16\}$}
    \nonl
    \myinput{Optimized wordlenght vector $\mathbf{b}^{\text{sel}}$}
    \nonl
    \myinput{Reference quality $q_{\text{ref}}$ (PSNR in dB or SSIM in $[-1,1]$)}
    \nonl
    \myinput{Quality drop tolerance $\epsilon$}
    \KwOut{Quantized model $m_q$}
    \nonl\;
    
    
    $\mathbf{b}^{\text{sel}} \leftarrow \textbf{QuantSR-WLopt}(m, \mathcal{W}, q_{\text{ref}}, \epsilon)$ \\
    $\mathbf{q}^{\text{drop}}_{\text{sorted}}, \mathcal{L}_{\text{drop}}^{\text{sorted}} \leftarrow \textbf{LRA}(m, \mathcal{W}, q_{\text{ref}})$ \\
    $m_q^{\text{DRE}} \leftarrow \textbf{DREsel}(m(\mathbf{b}^{\text{sel}}), \mathbf{q}^{\text{drop}}_{\text{sorted}}, \mathcal{L}^{\text{sorted}}_{\text{drop}})$
    
    \caption{\footnotesize NPU-Aware Quantization for SR (NAWQ-SR)}
    \label{alg:nawq-sr}
\end{algorithm}


==> algorithms/wlopt.tex <==

% NPU-centric Hybrid-Precision Wordlength Optimization (QuantSR-WLopt)

\setlength{\textfloatsep}{0pt}
\SetArgSty{\textnormal}
\begin{algorithm}[!t]
    \footnotesize
    \SetAlgoLined
    \LinesNumbered
    \DontPrintSemicolon
    \KwIn{DNN $m$ with layers $\mathcal{L}$, Wordlengths set $\mathcal{W}=\{8,16\}$}
    % \nonl
    % \myinput{Wordlengths set $\mathcal{W}=\{8,16\}$}
    \nonl
    \myinput{Quality drop $q_{\text{w-quant}}^{\text{drop}}$  of 8-bit weights-quantized DNN}
    \nonl
    \myinput{Reference quality $q_{\text{ref}}$ (PSNR in dB or SSIM in $[-1,1]$)}
    \KwOut{Sorted layers with respect to quality drop $\mathcal{L}^{\text{sorted}}_{\text{drop}}$}
    \nonl
    \myoutput{Sorted layerwise quality drops $\mathbf{q}^{\text{drop}}_{\text{sorted}}$}
    % \nonl\;
    $q_{\text{ref}} \leftarrow q_{\text{ref}} -     q_{\text{w-quant}}^{\text{drop}}$ \tcp*[f]{\scriptsize Remove quality drop due to 8b weights}  \\
    $u \leftarrow$ uniform wordlength (in our case 16 bits) \\ 
    % $\mathbf{b}_l \leftarrow u \quad \forall l \in \{0, ..., |\mathcal{L}|-1\}$\\

    \ForEach( \tcp*[f]{\scriptsize for each layer}){$l$ \textbf{in} $\mathcal{L}$} {
        $\mathbf{w} \leftarrow \mathbf{u}$ \\
        $w_l \leftarrow 8$ \\
        $q \leftarrow \text{GetQuality}(m(\mathbf{w}))$ \\
        $\mathbf{q}^{\text{drop}}_l \leftarrow q_{\text{ref}} - q$ \\
    }
    $\mathbf{q}^{\text{drop}}_\text{sorted}, \mathcal{L}^{\text{sorted}}_{\text{drop}} \leftarrow \text{SortDescending}(\mathbf{q}^{\text{drop}})$ 
    
    % \footnotesize
    % \SetAlgoLined
    % \LinesNumbered
    % \DontPrintSemicolon
    % \KwIn{DNN $m$ with layers $\mathcal{L}$, Wordlengths set $\mathcal{W}=\{8,16\}$}
    % % \nonl
    % % \myinput{Wordlengths set $\mathcal{W}=\{8,16\}$}
    % \nonl
    % \myinput{Calibration set $\mathcal{D}_{\text{calib}}$}
    % \nonl
    % \myinput{Reference quality $q_{\text{ref}}$ (PSNR in dB or SSIM in $[-1,1]$)}
    % \nonl
    % \myinput{Quality drop tolerance $\epsilon$}
    % \KwOut{Optimized wordlength vector $\mathbf{b}^{\text{sel}} \in \mathcal{W}^{|\mathcal{L}|}$}
    % % \nonl\;
    % $u \leftarrow$ uniform wordlength (in our case 16 bits) \\ 
    % $b_l \leftarrow u \quad \forall l \in \{0, ..., |\mathcal{L}|-1\}$ \\
    % InitScales\&ZeroPoints($m(\mathbf{b})$, $\mathcal{D}_{\text{calib}}$)\\
    
    % $c^{\text{bops}}_{\text{total}}, \mathbf{c}^{\text{bops}}_{\text{layers}} \leftarrow \text{GetBOPs}(m(\mathbf{b}))$ \Comment{\scriptsize Initial cost} \\
    
    % $\mathbf{c}^{\text{sorted}}_{\text{layers}}, \mathcal{L}^{\text{sorted}}_{\text{bops}} \leftarrow \text{SortDescending}(\mathbf{c}^{\text{bops}}_{\text{layers}})$ \\
    
    % $\mathbf{b}^{\text{sel}} \leftarrow \mathbf{b}$ \\

    % \ForEach(\Comment{\scriptsize Single-shot pass through the layers}){$l$ \textbf{in} $\mathcal{L}^{\text{sorted}}_{\text{bops}}$}{}
    % \ForEach{}{}
        % $\mathbf{b} \leftarrow \mathbf{b}^{\text{sel}}$ \\
        % $b_l \leftarrow 8$ \\
        % UpdateScale\&ZeroPoint($b_l$) \Comment{\scriptsize Using Eq.~(\ref{eq:scale_factor})} \\
        % $q \leftarrow \text{GetQuality}(m(\mathbf{b}), \mathcal{D}_{\text{calib}})$ \\
        % $c^{\text{bops}} \leftarrow \text{GetBOPs}(m(\mathbf{b}))$ \\
        % \If(\Comment{\scriptsize Quality constraint}){$q_{\text{ref}} - q \le \epsilon$}{
        %     $\mathbf{b}^{\text{sel}}_{l} \leftarrow 8$ \\
        %   $q_{\text{best}} \leftarrow q$, \qquad $c^{\text{bops}}_{\text{min}} \leftarrow c^{\text{bops}}$ \\ 
        % }
    % }
    \caption{\footnotesize Wordlength \mbox{Optimization} (\textbf{QuantSR-WLopt})}
    \label{alg:static_wl_opt_refined}
\end{algorithm}


==> sections/10_revisions.tex <==
xThis document details the changes made to address all the major concerns from the reviewers of the previous MobiCom 2021 submission. 

\noindent
\textbf{Concern 1: PSNR gain is seemingly too small.}
Majority of the reviewers pointed out the marginal PSNR gain of 0.1 is not significant and that PSNR does not always reflect visual quality well. We agree and add more visual comparisons to the paper to show that this marginal PSNR drop can introduce undesirable visual artifacts, placing a heavier emphasis on the \textbf{qualitative} impact of INT8 quantization in super-resolution. We also further explain that although small changes in the value of the pixels due to quantization would result in minor differences in the pixel-to-pixel distance with respect to their ground-truth, these small changes can collectively introduce perceptually significant irregularities in texture and color. Instead, NAWQ-SR achieves both faster execution and quality that is perceptually evidently higher.

\noindent
\textbf{Concern 2: Exploring NPU for SR is not new.}
Some reviewers commented that previous frameworks such as MobiSR have already utilized the NPU. We further clarify that previous SR works naively utilize the NPU, leading to significant visual degradation due to the \textit{1)}~quantization impact of INT8 (Concern~1) and \textit{2)}~suboptimal deployment of the upsampling layers (Concern~4). For instance, MobiSR dispatches fewer patches to the NPU - partly alleviating its impact on quality, but increasing the latency by excessively falling back to CPU/GPU - and NEMO avoids using the NPU entirely in order to meet acceptable visual quality. To the best of our knowledge, our work remains the first to introduce the novel algorithms and components needed to mitigate the bottlenecks of utilizing the NPU for on-device super-resolution. 

\noindent
\textbf{Concern 3: Comparisons with previous SR frameworks are not fair.}
%  - Comparison to MobiSR shows gain but it is unclear whether the gain is from the dynamic quantization or different hardware mapping or other misc. optimizations (4.4). If the main technique (dynamic quantization) is not the main contributor of the gain (it seems the case), it is not a fair/insightful comparison.
%  - Comparison with MobiSR SplitSR is not to the point (orange and apple) -- they use or primarily use CPU/GPU.
Another major concern mentioned in the reviews was that the comparisons of our framework, as a standalone system, with MobiSR and SplitSR were unfair as these systems primarily use CPU/GPU. 
We re-emphasize in the evaluation section of our newly revised paper that we are comparing these systems as separate state-of-the-art solutions for on-device super-resolution as originally proposed by the respective authors in order to hit the recommended accuracy-latency trade-offs. In particular, in the current submission, we clarify that MobiSR and SplitSR constitute the start-of-the-art image SR systems using \textit{1)}~heterogeneous processors and \textit{2)}~CPU, respectively. We also highlight that we re-implemented MobiSR on the same device in order to achieve a fair comparison. Note that MobiSR rarely uses the NPU in order not to penalize quality and hence it predominantly uses the CPU/GPU; forcing MobiSR to primarily use the NPU would have been an unfair comparison as it would violate its quality threshold (Concern~2), leading to even bigger gains from using our approach. As described in the paper (Section 5.4), we tune the total-variation threshold of MobiSR (which determines the allocation of patches across CPU/GPU/NPU) in order to provide the highest-performing configuration for each experiment and obtain a very strong baseline against NAWQ-SR.

Furthermore, we added a comparison to XLSR, an on-device super-resolution system that got published since our last submission. XLSR is the winning system of the 2021 MAI challenge for mobile NPU-based super-resolution, which was co-located with CVPR 2021, and represents the current state-of-the-art of \textit{3)}~NPU-based super-resolution. In Section 5.4, we show that our framework achieves higher visual quality than XLSR, while achieving 91\% lower latency.

\noindent
\textbf{Concern~4: Comparisons with INT8-NPU}
% 8-bit computation is sufficient for many applications.
% - It is not surprising to see that the system in the end mostly utilize just 8-bit computations with occasional dynamic quantization for scaling. It is widely believed that 8-bit computation (as in Google TPU) is sufficient for many applications. Attaining the performance of 8-bit-only processing without loosing accuracy is the high level contribution of this paper, which is not particularly notable.  
Some reviewers have the misconception that 8-bit computations are sufficient in super-resolution as they are in many other DNN applications. Hence, attaining the latency of INT8 without losing much accuracy is not particularly notable. In our revised paper, we aim to clarify that misconception through \textit{1)}~visual comparisons (Fig.~1) (Concern~1) and \textit{2)}~a discussion on the lack and underutilization of NPU adoption in previous on-device super-resolution frameworks (Concern~2). 
% To this end, we change our INT8-NPU baseline in all our evaluations to reflect the current status-quo in deploying super-resolution models on the NPU. Notably, our previous INT8-NPU baseline reflects the theoretical latency speed-ups when all layers in the model are supported. However, in practice, current NPU support for efficient upsampling layers such as pixel shuffle, as acknowledged by previous works such as NEMO, are not supported, leading to the use of more expensive alternative layers such as transpose convolutions. Our new INT8 baseline reflects this additional computation, which is counteract by our proposed neural image codec. This results in a XX speedup...

\noindent
\textbf{Concern~5: Evaluation of DRE layer selection method:}
Lastly, some reviewers were unclear about how well our method for selecting the DRE layers (Section 4.2) would perform against a random selection approach. In response, we added random layer selection for dynamic quantization, RandDRE, as a baseline to further highlight the advantages of DRE. As detailed in our evaluation of DRE in the revised paper, RandDRE uses NAWQ-SR's selected bitwidths for each layer and uniform probability to randomly select the number of DRE layers and then randomly select the layers. This suboptimal selection of layers result in a 19.5$\times$ average higher overhead than using DRE, which automatically determine both the number and the DRE layers in a single step. We also re-emphasize that the gains of DRE is attributed to smart selection of layers according to cumulative layer energy, which is the indicator of a layer’s sensitivity to low precision and its impact on image quality, starting from the most expensive layer.


% \textbf{Motivations of Dynamic Range Estimation (DRE)}
% %  - Comparison to MobiSR shows gain but it is unclear whether the gain is from the dynamic quantization or different hardware mapping or other misc. optimizations (4.4). If the main technique (dynamic quantization) is not the main contributor of the gain (it seems the case), it is not a fair/insightful comparison.
% % Just as importantly, the paper did not go into the details as to why NAWQ-SR achieves accuracy close to always using A16W8 but latency close to always using  INT8.The later suggests it chose INT8 for most of the layers (or FLOP count), but the former suggests the few layers using A16M8 somehow made a huge different. What layers are these and why do they matter so much to the accuracy (while the rest layers don't)?
% Lastly, some reviewers were unclear about the gains of the dynamic range estimation (DRE) module. In response, we added random layer selection for dynamic quantization, RandDRE, as a baseline to further highlight the advantages of DRE. As detailed in our evaluation of DRE in the revised paper, RandDRE uses NAWQ-SR's selected bitwidths for each layer and uniform probability to randomly select the number of DRE layers and then randomly select the layers. This suboptimal selection of layers result in a 19.5$\times$ average higher overhead than using DRE, which automatically determine both the number and the DRE layers in a single step. We also re-emphasize that the gains of DRE is attributed to smart selection of layers according to cumulative layer energy, which is the indicator of a layer’s sensitivity to low precision and its impact on image quality, starting from the most expensive layer.



% Other stuff that reviewers commented but I did not include in this revision

%  - Dynamic quantization parameter adaptation is nothing but a form of batch normalization. It adjusts the scaling parameter in quantization based on value distribution before quantization. So the overall optimized mode is 8-bit quantization + batch normalization for scaling in a nutshell. 

%  - Algorithms 1, 2, 3 are ok but not particularly insightful. Those are rather standard heuristic-based algorithms to determine quantization levels. 

==> sections/old_1_introduction.tex <==



\vspace{-0.4cm}
\section{Introduction}
\label{sec:intro}
\vspace{-0.15cm}

With the rapid rise of Internet content delivery services and devices that support higher resolution content, images and videos are predicted to account for 82\% of the global Web traffic~\cite{ciscovni}. 
Mobile applications, in particular, constitute a great proportion of this growth, as services such as live streaming, video-conferencing, and video-on-demand have been on the rise. 
For instance, popular video application TikTok has over 50 million daily users and has seen a 55\% increase in unique users and a 93.7\% increase in the average time spent per user in just six months~\cite{tiktok_stats}. 
Additionally, with more than half of U.S. Gen Z population on Snapchat, the messaging app 
%had a total of 
reached 249 million daily users in Q3 of 2020, resulting in 
%a 25\% growth in the average number of content created and 
a 50\% growth of daily time spent watching content year-over-year~\cite{snapchat_stats}. 
Therefore, in order to meet these demands, existing mobile systems are required to maximize both the user satisfaction and their quality of experience (QoE).

A primary challenge of this class of mobile systems is their sensitivity to networking conditions. Due to the large amount of transferred data and the stringent latency constraints, the quality of the communication channel between client and server plays a key role in satisfying the app-level performance needs. Nevertheless, in real-world cellular networks, the network speed fluctuates substantially, and poor connectivity conditions lead to excessive response times, dropped frames or video stalling, which rapidly degrade the QoE~\cite{videoqoe2011inm,videoqoe2009itng,videoqoe2016imc,Yin2015sigcomm}. This phenomenon is further aggravated by the increasing number of users which compete for the same pool of network resources and create contention~\cite{netpolice2009imc}.

For many years, adaptive bitrate (ABR) has been the dominant approach to remedy this situation, ending up in large-scale deployments, such as Netflix~\cite{abrnetflix2019mmsys}, YouTube~\cite{abryoutube2020pam}, and Hulu~\cite{abrhulu2012imc}.
ABR methods typically operate by considering either the network speed or the playback buffer state and selecting accordingly the bitrate of the downloaded media, either in a per-segment manner for videos or per frame for images~\cite{Mao2017,Guan2020,Du2020,Gadaleta2017}. 
Although ABR approaches have boosted the performance of existing %content delivery 
systems, there is still substantial room to further optimize the bandwidth usage~\cite{abryoutube2020pam,neuroabr2020jsac}.

A recent key method with the potential to push beyond ABR's performance is \textit{neural enhancement}, enabled through super-resolution (SR) deep neural networks (DNNs)~\cite{SRCNN}. 
SR DNNs operate by processing a low-resolution, degraded image and automatically generating a high-quality, high-resolution output. This allows low-quality content to be transmitted across the network, at the expense of additional computation at the receiver's end.
Hence, neural enhancement removes the system's sole reliance on the network and opens up a new dimension in the design space by introducing a trade-off between the use of network and computational resources~\cite{neuralenhancementcds2020}.
Naturally, these approaches can be utilized alongside image and video compression techniques and ABR algorithms, resulting in their integration in a plethora of content delivery systems~\cite{video_delivery2017hotnets, analytics20192019, live_streaming2020sigcomm, 360stream2020infocom}.

Even so, deploying these neural enhancement-based techniques on mobile devices still remains an active challenge.
Despite the increasing computational capacity of mobile devices, executing SR models is still excessively demanding with respect to both workload and memory.
For instance, due to the upscaling nature of SR models, the number of multiply-add operations required even for efficient mobile-tailored SR DNNs is orders of magnitude larger than their discriminative counterparts~\cite{mobisr2019mobicom}.
In order to counteract the excessive computational requirements, existing systems \textit{1)}~rely on floating-point implementations, such as assuming the availability of a desktop GPU client~\cite{video_delivery2018osdi, dejavu2019hotmobile}, \textit{2)}~require the use of all available processors (CPU, GPU, DSP) in parallel~\cite{mobisr2019mobicom}, \textit{3)}~leverage frame dependencies in order to cache previously upscaled results~\cite{nemo2020mobicom} or \textit{4)}~resort to cloud offloading~\cite{supremo2020tmc}.

Nevertheless, these solutions are either limited in each deployment setting, and thus cannot accommodate a wide range of heterogeneous low-end devices, or introduce additional challenges as a by-product.
Specifically, using multiple compute engines in parallel~\cite{mobisr2019mobicom} can result in thermal throttling issues~\cite{mitra2016dac,mitra2019tcad,fire_in_your_hand2019mobicom} and cached-based solutions can lead to a drastic drop in visual quality~\cite{nemo2020mobicom,supremo2020tmc}.
More importantly, offloading approaches~\cite{supremo2020tmc} exacerbate the bandwidth usage, defeating the purpose of utilizing these models. 
Therefore, there is a need for novel solutions that enable the use of SR DNNs on mobile devices without incurring any of the aforementioned drawbacks.


In this work, we present \tool, a framework that overcomes the limitations of existing on-device SR systems and delivers fast, efficient and high-quality SR on mobile.
To optimize %the attainable 
latency while meeting the user-specified quality constraints,
\tool adopts an NPU-centric approach, introducing a novel \textit{hybrid-precision execution} paradigm and a runtime \textit{neural image codec} that exploit the multi-precision processing capabilities of modern mobile NPUs. 
Moreover, we propose a mechanism that selectively re-customizes on-the-fly the arithmetic precision of the DNN layers, improving visual quality beyond the state-of-the-art NPU-based designs.
This paper makes the following key contributions:
% \vspace{-0.1cm}
\begin{itemize}[leftmargin=*]
    \item A novel hybrid-precision execution scheme together with a methodology for optimizing the deployment of SR DNNs to the latency and quality requirements of the target application.
    By considering the multiple precisions supported by a given NPU, our framework adapts each layer's wordlength through a single-shot optimization algorithm, co-optimizing the per-layer quantization of the DNN and the scheduling of its layers on the NPU. 

    \item A novel technique that identifies quantization-sensitive layers and selectively applies adaptive arithmetic precision, enhancing them with wider representational power at run time. This technique dynamically adapts the quantization parameters of the selected layers in an input-dependent manner, leading to lower quantization error and higher visual quality than previously attainable on mobile NPUs. 
    
    \item To the best of our knowledge, this work is the first SR approach to exploit the multi-precision capabilities of the heterogeneous processing units that reside in NPUs.  
    To this end, we propose a new neural image codec design comprising a hybrid-precision dispatcher and a run-time quantization unit. 
    % Our neural image codec 
    The module is configured with the SR DNN-optimized hybrid-precision configuration and the associated execution schedule, delivering an average speedup of 7.3$\times$ over the state-of-the-art on-device SR systems.
\end{itemize}


% Hybrid-precision execution + Wlopt
% LRA + DRE
% NIC + NPU and speedups


% \item In order to efficiently utilize the underlying hardware, we adopt a layerwise multi-wordlength quantization approach. Each layer's wordlength is adapted through our novel single-shot optimization algorithm that consistently outperforms popular heuristic optimizers under the same search time budget, leading to significant gains in both computation and memory requirements.
    

==> sections/old_2_background_rw.tex <==

\vspace{-0.15cm}
\section{Background \& Related Work}
\label{sec:background}
\vspace{-0.15cm}

The unprecedented performance of SR DNNs in restoring realistic textures has made them a key component behind a broad range of products and use-cases, from high-resolution TVs~\cite{samsung_tv_ai_upscaling} to gaming GPUs~\cite{nvidia_dynamic_sr}.
%has seen this technology becoming adopted
% The successful adoption of DNNs for SR~\cite{SRCNN} has demonstrated unprecedented performance in restoring realistic textures, resulting in naturally pleasing images.
As a result, 
% Since then, there have been a wide variety of works that
several works have focused on different aspects of improving the performance of SR models, investigating their architecture~\cite{RCAN, IDN}, the training methodology~\cite{SRGAN, ESRGAN}, and the augmentation of training data~\cite{suppressingmocvprworkshop2019, rethinkdataaugyoocvpr2020}. 
%, in order to push the performance of these models.
Although significant progress has been made in mapping low-resolution (LR) images closer to their high-resolution (HR) counterparts~\cite{USRNet, DAN}, 
%the efficiency of these high-end performing models is still lacking; 
SR DNNs still have excessive computational and memory demands.
As such, they are not viable for most real-world mobile deployments.
% , which in turn are not viable for most real-world mobile deployments.

\textbf{Efficient Super-resolution.}
% In order to improve the efficiency of SR models, recent works have proposed specialized model architectures either through manual design~\cite{IDN, CARN, IMDN} or neural architecture search (NAS)~\cite{tpsr2020eccv, FALSR, ESRN}.
Recent works have proposed efficiency-optimized model architectures, either through manual design~\cite{IDN, CARN, IMDN} or neural architecture search (NAS)~\cite{tpsr2020eccv, FALSR, ESRN}.
Prominent hand-crafted works have presented optimizations to avoid computing large feature maps~\cite{SRCNN} and mitigate the cost of upscaling through the use of pixel-shuffle layers~\cite{ESPCN,FEQE}.
%ong \textit{et al.}~\cite{SRCNN} first proposed reconstructing the LR image at the very end of the DNN to avoid computing large feature maps during feature extraction. 
%Towards mitigating the upscaling cost, Shi \textit{et al.}~\cite{ESPCN} proposed the pixel-shuffle operation as an efficient upscaling alternative to the computationally expensive transpose convolution. 
%Similarly, the idea can also be applied to downsample the input LR image to further reduce the complexity through an inverse operation of the pixel shuffle which was first utilized in~\cite{FEQE} for SR.
Another line of work focused on replacing convolutions with more efficient blocks, such as CARN's group convolutions~\cite{CARN} and IMDN's channel splitting~\cite{IDN,IMDN}.
% Besides the innovation in overall network design, numerous works aimed to reduce the complexity of the convolution operation through tensor decomposition and other more efficient architectural substitutes. 
% For instance, Ahn \textit{et al.}~\cite{CARN} adopted group convolutions~\cite{resnet} and Hui \textit{et al.}~\cite{IDN, IMDN} proposed IDN and subsequently IMDN which utilizes channel splitting~\cite{shufflenetv2} to skip the computation of a subset of feature maps.

Apart from manual efforts, NAS has also been a popular approach in designing efficient SR models.
%and has largely found success in optimizing hardware-aware models~\cite{Liu_2018_ECCV, NPENAS2020, 1912.00848, MnasNet_2019, FBNet_2019, latbenchnips2020}.
% Specifically for SR, 
Chu \textit{et al.}~\cite{MoreMNAS, FALSR} proposed a search on a multi-objective optimization function, targeting image fidelity, compute, and memory, using  reinforcement learning and evolutionary methods.
Song \textit{et al.}~\cite{ESRN} minimized the search time by considering hand-crafted residual building blocks, 
% which were commonly designed and used for SR, 
instead of searching for more primitive operations.
More recently, Lee \textit{et al.}~\cite{tpsr2020eccv} proposed a generative adversarial network (GAN) search and found a tiny model, named TPSR, that can focus on maximizing either image fidelity or perceptual quality.
Despite the algorithmic advances, the on-device execution of these models is still impractical for real-world mobile devices, resulting in numerous system-based solutions~\cite{neuralenhancementcds2020} that aim to enable these models to be efficiently and effectively deployed.

\textbf{On-device Super-resolution.}
The primary paradigm of using SR on mobile phones comprises the transmission of compact LR images, followed by their upscaling and visual quality recovery on the device through an SR DNN~\cite{video_delivery2017hotnets}. In this manner, the transfer load is minimized, drastically reducing the bandwidth requirements and the corresponding cellular data cost for both the users and the service provider.  %, with the visual quality recovered on the smartphone side.
Such applications span from video-on-demand~\cite{video_delivery2018osdi} and video-conferencing~\cite{dejavu2019hotmobile}, to graphics enhancement in mobile game streaming~\cite{stadia2021} and data-saving alternatives of image-centric social media apps, such as Facebook Lite.

Towards deploying SR models on mobile devices, the state-of-the-art on-device SR frameworks~\cite{mobisr2019mobicom, supremo2020tmc,nemo2020mobicom,splitsr2021imwut} have adopted different approaches. 
One line of work~\cite{mobisr2019mobicom,supremo2020tmc} has focused on utilizing the heterogeneous processors (\textit{e.g.}~CPU, GPU, NPU) found in many recent devices. 
In order to effectively load-balance across these processors, these systems exploit the observation that patches of an image have varying upscaling difficulty. 
For instance, MobiSR~\cite{mobisr2019mobicom} adopts a total-variation metric to quantify the upscaling difficulty of each patch, which is then used for scheduling.
Besides scheduling, the video-focused NEMO~\cite{nemo2020mobicom} leverages the inter-frame dependencies in order to cache and reuse previously super-resolved patches, resulting in considerable speedup without consuming excessive energy.
Finally, SplitSR~\cite{splitsr2021imwut} combined lightweight model design with compiler optimizations to improve CPU-based SR.

Even though these frameworks enable fast on-device upscaling, they come at the high cost of quality degradation. 
Notably, deploying these models on compute engines that run on lower bitwidths, such as DSPs and NPUs, causes a considerable drop in visual quality as seen in recent SR mobile systems such as MobiSR~\cite{mobisr2019mobicom} and NEMO~\cite{nemo2020mobicom}.
As a result, existing systems either reduce the number of patches dispatched to these compute engines~\cite{mobisr2019mobicom} or entirely avoid using them~\cite{nemo2020mobicom,splitsr2021imwut}.
As little work has been done to mitigate the effects of quantization on SR models, our work aims to breach this gap to allow existing 
%algorithmic-based and system-based %
techniques to leverage the full capabilities of modern 
%low-bitwidth 
NPUs that can be found across commodity smartphones~\cite{embench2019emdl,ai_benchmark2019iccvw,snpe,arm_ethos_npu}.
\stelios{We could say that their performance is limited by the higher-precision compute engines.}

\textbf{Reduced-precision Quantization.}
Beyond SR, precision quantization constitutes a prominent method for minimizing the computational and memory demands of DNNs.
State-of-the-art quantization approaches~\cite{qcnns2016cvpr,int_only2018cvpr} typically adopt block floating-point schemes (also known as dynamic fixed-point), where a value $x$ is quantized as $x_{\text{quant}} = \left\lfloor x \cdot s_l - z_l \right\rceil$ using a \textit{uniform} wordlength\footnote{We use the terms \textit{wordlength} and \textit{bitwidth} interchangeably.} $b$ across all layers and with different scale factors $s_l$ and zero points $z_l$ for each layer $l$.
The majority of existing works either \textit{1)}~apply quantization to already trained 32-bit full-precision models, followed by a retraining step to fine-tune the DNN's weights~\cite{ristretto2018tnnls,angeleye2018tcad}, or \textit{2)}~perform quantization-aware training to directly obtain low-precision models~\cite{qcnns2016cvpr,int_only2018cvpr}. As such, both approaches involve a computationally expensive training step.
% However, both approaches require the availability of training data which is not always a realistic assumption in real-world scenarios~\cite{private_dl2015ccs}, such as for datasets collected by commercial companies that remain proprietary or reveal private information of users~\cite{gdpr2018}. \manote{we need to say that even without retraining we achieve significant visual quality. bound it and comment on cost.}

At the same time, although various quantization methods have been successfully applied on \textit{classification} DNNs without incurring significant accuracy loss~\cite{int_only2018cvpr}, these do not generalize to SR models, often leading to a catastrophic drop in visual quality~\cite{mobisr2019mobicom,nemo2020mobicom,PAMSQS}.
% As shown in~\cite{mobisr2019mobicom,PAMSQS}, directly transferring classification-tailored quantization methods to SR DNNs leads to a catastrophic drop in visual quality. 
This is primarily due to the fact that Batch Normalization (BN) layers have been removed from state-of-the-art SR models~\cite{RCAN,tpsr2020eccv,IMDN} as they were shown to severely restrict their representational power~\cite{EDSR}. 
In turn, the absence of BN layers leads to significant variability in the dynamic range of activations, making the direct utilization of 
%state-of-the-art 
quantization methods futile~\cite{int_only2018cvpr} or requiring expensive architectural modifications and retraining~\cite{efficientbnnsrMa2019,bnnsrXin2020,PAMSQS}.

Hence, with the increasing integration of low-precision NPUs on smartphones, there is an emerging need for novel quantization techniques that are particularly crafted for on-device SR, combining high quality with efficiency. 
% models in order to efficiently deploy them on mobile devices. % without degrading quality
%In this context, \tool alleviates the need for an excessively expensive (re-)training process.
In this context, %Through a number of novel techniques, 
our \tool framework introduces novel \textit{post-training} techniques that closely approach the quality of full-precision models, leaving little room for improvement through expensive retraining.
% Instead, an NPU-aware multi-wordlength quantization method is introduced, together with a layer-selective run-time precision adaptation mechanism. These techniques allow \tool to closely approach the quality of full-precision models, leaving little room for improvement through expensive retraining. 
In addition, \tool
% c
% 's post-training approach 
can be applied complementarily on models that have been trained in a quantization-aware manner.

% In this context, \tool alleviates the need to access the whole training set, as it does not involve model training. Instead, an NPU-aware multi-wordlength quantization method is introduced together with a layer-selective run-time quantization mechanism. These two techniques lead to SR DNNs that can be efficiently executed on mobile NPUs while also sustaining high visual quality.

\textbf{Challenges and Opportunities of NPUs.}
Recently, vendors have been integrating dedicated NPUs into their mobile devices~\cite{embench2019emdl,ai_benchmark2019iccvw}. 
Designed explicitly to provide fast and efficient execution of DNN workloads, NPUs typically consist of highly optimized low-precision processing units for convolution and matrix operations.
These units provide higher energy efficiency than CPUs and GPUs by omitting general-purpose hardware logic, increasing at the same time the availability of computational resources for other tasks by taking over the compute-intensive DNN execution. 
Despite their benefits, NPUs can often lead to degraded output quality compared to their full-precision counterparts, as data are represented using 16- or 8-bit fixed-point precision~\cite{snpe,arm_ethos_npu}. 

% Nevertheless, 
Recent hardware advances have led to NPUs that support \textit{multiple arithmetic precisions}~\cite{snpe,arm_ethos_npu,huawei_npu2019hotchips}. Such examples are the Hexagon 698 processor on Qualcomm Snapdragon 865 (SDM865)~\cite{snpe} and the Arm Ethos processor~\cite{arm_ethos_npu}, both supporting two precision modes: 8-bit for both activations and weights (INT8) or 16-bit for activations and 8-bit for weights (A16W8). 
In spite of the new opportunities of these hardware architectures, existing deployment methodologies fail to exploit them.
As such, current approaches lead to \textit{1)}~fast but low-quality execution (INT8 - due to the quantization-induced error), \textit{2)}~higher quality but slow execution (A16W8 - close to 2$\times$ slower than INT8, as shown in Section~\ref{sec:eval_baselines}), or \textit{3)}~slow and low-quality execution (A16W8) for models where even existing 16-bit quantization methods do not suffice - which is often the case for SR models. 
Our work pushes the boundaries of what is possible in terms of mapping SR models to NPUs, yielding fast and high-quality designs that fully utilize their multi-precision processing capabilities.


% As mentioned in \stelios{the Related Work section}, there are several methods for finding the optimal quantization configuration for a given model.
% These schemes typically proceed by calculating the sensitivity of a given layer to quantization by evaluating how small disturbances within that layer influence the end quality of result (QoR), \textit{i.e.}~accuracy for classification tasks or image quality for enhancement and super-resolution tasks.
% Such approaches only focus on maximizing the model's accuracy... 
% However, when deploying DNNs on mobile and embedded devices, resources are limited and shared between multiple concurrent applications~\cite{nestdnn2018mobicom}.
% This is for instance the case in smartphones, where a single SoC is used to run multiple different applications~\cite{nestdnn2018mobicom,gables2019hpca}, or in mobile robots where multiple perceptual tasks, such as obstacle avoidance or human detection, are happening in parallel~\cite{traildnn2017iros,weights_virt2020mobisys}. In these cases, the desired QoR and the computational constraints of the model in question are known \textit{a priori}. Therefore, it is crucial to optimize the quantization configuration by considering both the model's QoR and workload. \manote{instead of workload should be hardware characteristics}
% \manote{tie sending only lr to reduced stalling and better QoE.}
% ....
